Exact and Approximated Log Alignments for Processes with Inter-case Dependencies

The execution of different cases of a process is often restricted by inter-case dependencies through e.g., queueing or shared resources. Various high-level Petri net formalisms have been proposed that are able to model and analyze coevolving cases. In this paper, we focus on a formalism tailored to conformance checking through alignments, which introduces challenges related to constraints the model should put on interacting process instances and on resource instances and their roles. We formulate requirements for modeling and analyzing resource-constrained processes, compare several Petri net extensions that allow for incorporating inter-case constraints. We argue that the Resource Constrained $\nu$-net is an appropriate formalism to be used the context of conformance checking, which traditionally aligns cases individually failing to expose deviations on inter-case dependencies. We provide formal mathematical foundations of the globally aligned event log based on theory of partially ordered sets and propose an approximation technique based on the composition of individually aligned cases that resolves inter-case violations locally.

==> 2_preliminaries/2_preliminaries_dep.tex <==
%%%%%%%%%%%%%%
% DEPRECATED %
%%%%%%%%%%%%%%


% In this section we present the notations that we will use throughout the paper.

% \subsection{Multisets and posets}





% \begin{definition}{(Multiset)} A multiset $m$ over a set $X$ is $m: X \rightarrow \Nat$. The set of all multisets over $X$ is denoted as $X^\oplus$. We define the support $\supp(m)$ of a multiset $m$ as the set $\{x \in X \mid m(x) > 0\}$. We write $|x|$ for $m(x)$, when it is clear from context that $x \in \supp(m)$.

% For two multisets $m_1,m_2$ over $X$, we write $m_1 \leq m_2$ if $\forall_{x \in X}: m_1(x) \leq m_2(x)$, and $m_1 < m_2$ if $m_1 \leq m_2 \wedge m_1 \neq m_2$. We define $m_1+m_2$ as $(m_1 + m_2)(x) =m_1(x) + m_2(x)$ for all $x\in X$. For  $m_1 \geq m_2$, we define  $m_1-m_2$ as  $(m_1 - m_2)(x) =m_1(x) - m_2(x)$ for all $x\in X$.

% We extend the standard set operations of union and intersection to multisets as follows. With two multisets $m_1,m_2$ over $X$, we write $m = m_1 \sqcup m_2$ if $\forall_{x \in X}: m(x) = \max(m_1(x), m_2(x))$ and $m = m_1 \sqcap m_2$ if $\forall_{x \in X}: m(x) = \min(m_1(x), m_2(x))$.
% \end{definition}

% In some cases we consider multisets over a set $X$ as vectors of length $|X|$, where we assume arbitrary but fixed orderings of elements of $X$.

% \begin{definition}{(Partial order)}
% A partial order over a set $E$ is a binary relation $\prec \subseteq E \times E$ that is (1) irreflexive, \ie $x \nprec x$, (2) antisymmetric, \ie $x \prec y \implies y \nprec x$ and (3) transitive, \ie $x \prec y \wedge y \prec z \implies x \prec z$. With $x,y \in E$, $x \| y$ denotes that $x \nprec y \wedge y \nprec x$.

% If it is not clear by context, we write $\prec_E$ denoting that $\prec$ is defined over the set $E$.

% The transitive closure $\prec_E^+$ of a partial order $\prec_E$ is defined by $\prec_E^+ = \prec_E \cup \set{ (a, c) | a, c \in E, \exists_{b \in E} a \prec_E b \prec_E c }$.
% \end{definition}

% \begin{definition}{(Partially ordered set)}
% A \emph{partially ordered set}, also denoted as \emph{poset}, $X = (\bar{X}, \prec_X)$ is a pair of a set $\bar X$ and partial order $\prec$ over this set $\bar X$. We overload the notation by saying that $x \in X \implies x \in \bar X$.

% \tent{We extend the standard set operations of union, intersection and subset to posets as well.}

% An antichain $X' \subseteq X$ is a subposet of $X$ such that for every $x,x' \in X_1$ we have $x \nprec x'$ and $x' \nprec x$. The partial order is defined for antichains as well. With two antichains $X_1, X_2 \subseteq X$, we have $X_1 \prec X_2$ if and only if $\exists_{x_1 \in X_1, x_2 \in X_2} x_1 \prec x_2$. Furthermore, with $x \in X$, we have $x \prec X_1$ if and only if $\exists_{x_1 \in X_1} x \prec x_1$. Similarly, $X_1 \| X_2 \iff \forall_{x_1 \in X_1, x_2 \in X_2} x_1 \| x_2$ and $x \| X_1 \iff \forall_{x_1 \in X_1} x \| x_1$.

% The set of minimum elements of $X$, denoted by $\min(X)$, is an antichain $\min(X) \subseteq X$, such that $\min(X) = \set{x \mid x \in X, \forall_{x' \in X}: x' \nprec x }$. Similarly, $\max(X)$ is the set of maximum elements of $X$, \ie $\max(X) = \set{x \mid x \in X, \forall_{x' \in X}: x \nprec x' }$.

% A sequence $\sigma \in X^*$ is a totally ordered set with order $\prec_\sigma$, such that $\prec \subseteq \prec_\sigma$.
% \end{definition}


% \begin{definition}{(Interval, prefix and postfix in a poset)}\label{def:poset_interval}
% With a poset $X = (\bar X, \prec)$ and two antichains $X_1, X_2 \subseteq X$, a closed poset interval $\interval{X_1}{X_2}$ is the subposet containing all elements in $X$ between $X_1$ and $X_2$, including $X_1$ and $X_2$, \ie $\interval{X_1}{X_2} = (X_1 \cup X_2 \cup \set{x \mid x \in X, \exists_{a \in X_1} \exists_{b \in X_2} a \prec x \prec b }  )$. Furthermore, we define the open and half-open poset intervals as follows: $\intervalopen{X_1}{X_2} = \interval{X_1}{X_2} \setminus (X_1 \cup X_2)$, $\intervalhalfopenl{X_1}{X_2} = \interval{X_1}{X_2} \setminus X_1$ and $\intervalhalfopenr{X_1}{X_2} = \interval{X_1}{X_2} \setminus X_2$.

% Let $\bot$ and $\top$ be two elements such that for every element $x \in X$, $\bot \prec x \prec \top$. The half-open and open poset intervals $\prefix{X'}$ and $\prefixopen{X'}$ denoted by the prefix and open prefix of antichain $X' \subseteq X$.

% The union over two intervals $\interval{A}{B}$ and $\interval{C}{D}$, with antichains $A,B,C,D \subseteq X$, gives a set of disconnected intervals as follows:

% \begin{equation}
%     \interval{A}{B} \cup \interval{C}{D} =
%     \begin{cases}
%         \set{\interval{\min(A \cup C)}{\max(B \cup D)}} & \text{if } \interval{A}{B} \cap \interval{C}{D} \neq \emptyset \\
%         \set{\interval{A}{B}, \interval{C}{D}} & \text{otherwise}
%     \end{cases}
% \end{equation}
% Note that the intervals can also be either open or half-open.
% \end{definition}

% \begin{lemma}{(\todo{})}

% \end{lemma}

% \begin{definition}{(Projections on sets, multisets and posets)}
% Let $X$ and $Y$ be two sets or multisets. The projection from $Y$ on $X$, $X\proj_Y = X \cap Y$.

% With two posets $X = (\bar X, \prec_X)$ and $Y = (\bar Y, \prec_Y)$, $X\proj_Y = (\bar X \cap \bar Y, \prec_X \cap \prec_Y)$. Note that a set or multiset is a poset with $\prec = \emptyset$ and therefore the projection is also defined for $X\proj_Y$ with poset $X$ and set or multiset $Y$.
% \end{definition}


% \subsection{Petri nets}
% Petri nets can be used as a tool for the representation, validation and verification of workflow processes to provide insights in how the process behaves \cite{peterson1981petri}. 

% \begin{definition}{(Petri net)}
% A \emph{Petri Net} \cite{murata1989petri} is a 3-tuple $N = \langle P, T, \F \rangle$, where $P$ is the set of places, $T$ is the set of transitions, $P \cap T = \emptyset$, $\F: (P \times T) \cup (T \times P) \rightarrow \Nat$ is the flow of the net. The incidence matrix $F$ of a Petri net $N$ is a matrix with a row for each place $p\in P$ and a column for each transition $u\in T$ and it is defined by $F(p, u) = \F(u, p) - \F(p, u)$.

% We write $P(N)$, $T(N)$ and $\F(N)$ to indicate that we refer to the set of places, the set of transitions and the flow relation of a net $N$.

% $N_1 \cap N_2$, $N_1 \cup N_2$, and $N_1 \subseteq N_2$ denote intersection, union, and subsets of nets, respectively, defined on the sets of nodes and arcs of $N_1$ and $N_2$.

% A \emph{labeled} Petri net $N = \langle P, T, \F, \ell \rangle$ additionally defines a \textit{labeling} $\ell: T \rightarrow \Sigma^\bot = \Sigma \cup \{\tau\}$ assigning each transition $u$ a label $\ell(u)$ from alphabet $\Sigma$ or $\ell(u)=\tau$ for silent transitions. We assume that the intersection, union and subsets are only defined for two labeled Petri nets $N_1$, $N_2$ where $\ell_1(u) = \ell_2(u)$ for any transition $u \in T_1 \cap T_2$.
% \end{definition}

% \begin{definition}{(Post-set, Pre-set)}
% Given a transition $u \in T$, its \emph{pre-set} $\pre{u}$ and \emph{post-set} $\post{u}$ are multisets defined as follows: $\pre{u}(p) = \F(p,u)$ and $\post{u}(p) = \F(u, p)$ for $p \in P$. Correspondingly, for a place $p \in P$ we have $\pre{p}(u) = \F(u,p)$ and $\post{p}(u) = \F(p, u)$ for $u \in T$.
% \end{definition}

% \begin{definition}{(Marking)}\label{def:marking}
% A \emph{marking} $m: P \rightarrow \Nat$ of Petri net $N = \langle P, T, \F \rangle$ assigns how many tokens each place contains. A marking  defines the \emph{state of} $N$.
% \end{definition}

% \begin{definition}{(Enabling and firing of transitions, Reachable markings)}
% A transition $u \in T$ is \emph{enabled} for firing if and only if $m \geq \pre{u}$. We denote the \emph{firing} of $u$ by $m \xrightarrow{u} m'$, where $m'$ is the resulting marking after firing $u$ and is defined by $m' = m - \pre{u} + \post{u}$. For a transition sequence $\sigma = \langle u_1, \dots, u_m\rangle$ we write $m \xrightarrow{\sigma} m'$ to denote the consecutive firing of transitions $u_1$ to $u_m$. We also write $m \xrightarrow{*} m'$ if there is some $\sigma\in T^*$ such that $m \xrightarrow{\sigma} m'$.

% $\mathcal{M}(N)$ denotes the \emph{set of all markings}. The \emph{set of reachable markings} $\R(N, m)$ from marking $m$ in a Petri net $N$ is the set  $\{m'\mid  m \xrightarrow{*} m'\}$.
% \end{definition}


% \begin{definition}{(Place invariant)}
% A place invariant \cite{lautenbach1975liveness} is a row vector $I: P \rightarrow \mathbb{Q}$ such that $I \cdot F = 0$.  We denote the set of all place invariants as $\mathcal{I}_N$, which is a linear subspace of $\mathbb{Q}^P$. 
% \end{definition}

% The main property of place invariants is that for any two markings $m_1, m_2$ such that $m_1 \xrightarrow{*} m_2$ and any place invariant $I$ holds: $I \cdot m_1 = I \cdot m_2$.

% \begin{definition}{(Net system, Language, Execution sequence)}
% A \emph{Net system} is a tuple $SN = (N, m_i, m_f$), where $N$ is a Petri Net and $m_i$ and $m_f$ are respectively the initial and final marking. The \emph{language} of $SN$ is the set $\mathcal{L}(SN) = \{\sigma \in T^* \mid m_i \xrightarrow{\sigma} m_f \}$ of all  full firing sequences of $SN$.

% An \emph{execution sequence} in a net system $SN = (N, m_i, m_f)$ \tent{is a poset of steps}, starting at the initial marking $m_i$ and ending at the final marking $m_f$.
% \end{definition}


% \subsection{Event logs}
% An event log records action executions as events where each event records at least the action that occurred, the time of occurrence and the case identifier of the case in which the action occurred. Often resources are also recorded as event attributes, e.g. the actors executing the action. Typically, there are several types of resources, and it is generally known beforehand which resources of which types are involved in which actions.

% \begin{definition}{(Cases, Resources)}
% \tent{$\Idc$ denotes the \emph{set of case identifiers}. An identifier of case $c$ is denoted as $\idc$.}

% $R = \{r_1,\dots,r_m \}$ is the \emph{set of resource types}. Each resource instance with a name $\idr$ or $\idr_r$ belongs to some resource type $r \in R$. $\Idr$ denotes the multiset of resource instances of type $r \in R$. We assume that $\Idr \cap Id_{r'}=\emptyset$ for any $r,r' \in R$ with $r\neq r'$. $\IdR = \uplus_{r \in R} \Idr$ denotes the set of the resource instances of all types. 

% \end{definition}
% Note that if one would want to capture resource instances with multiple types $R' \subseteq R$, a new type should be constructed containing all types from $R'$.

% With the notation on cases, resources and resource types, we can define events, an event log and its traces in an abstract manner:

% \begin{definition}{(Event, Event log, Trace)}\label{def:event_log}
% An \emph{event} $e$ is a tuple $(a, ts, \idc, Id_R')$, with an activity $a = \act(e) \in \Sigma$, a timestamp $t = \etime(e) \in \mathbb{R}$, a case identifier $\idc = \ecase(e) \in \Idc$ and a multiset of resource instance identifiers $Id_R' = \Res(e) \leq \IdR$. Such an event represents that activity $a$ occurred at timestamp $t$ for case $\idc$ and is executed by resource instances from $Id_R'$ belonging to possibly different resource types.

% An event log $L$ is a (partially) ordered set of events with partial order $\prec_L$. These events can be split into traces, defined as projections e.g. on the case identifiers or on the resource names. For every $\idc \in \Idc$, $L_c$ denotes a trace projected on the case identifier $c$. $L_c = (\set{ e \mid e \in L, \ecase(e) = c }, \prec_{L_c})$, with $\prec_{L_c} = \set{ (e, e') \mid (e, e') \in \prec_L, \ecase(e) = \ecase(e') = c }$.
% %\tent{Also denoted as $\langle a_\idc^{Id_R'} \rangle$.?}
% \end{definition}

% For a process modeled by a Petri net, an activity name corresponds to a transition name or a transition label of the corresponding transition of a (labeled) Petri net.
% With the projection on case identifiers, we get the events from individual cases, as is mainly used in classical process mining and with projection on resource names, we can get the events from individual resource instances, which are entities in their own right, providing the perspective of a single or multiple resource types.


==> tables/extension_req.tex <==
\reducemargin{
\arraystretchtable{
\begin{table}[H]\caption{Satisfaction of requirements from Sec.~\ref{sec:req} by existing Petri net extensions.}\label{tab:extension_req}
\centering
\begin{tabular}{| l | c | c | c | c | c |}
\hline
& Disting. & Disting.     & Durable   &  Case-Res.   & Invertible \\
& cases    & resources    & resources &  Correlation & operations \\ \hline

RCWF-nets~\cite{van2006resource} 
 & \green{\checkmark} & \red{\xmark} & \green{\checkmark} & \red{\xmark} & \green{\checkmark} \\ \hline

$\nu$-Petri nets~\cite{rosa2010decision}
 & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \red{\xmark} & \green{\checkmark} \\ \hline

RIAW-nets~\cite{montali2016model} 
 & \green{\checkmark} & \red{\xmark} & \green{\checkmark} & \red{\xmark} & \green{\checkmark} \\ \hline

Synchronizing proclets~\cite{fahland2019describing}
 & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} \\ \hline

DB-nets~\cite{montali2017db}
 & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \red{\xmark} \\ \hline

CLog-nets~\cite{ghilardi2020petri}
 & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \green{\checkmark} & \red{\xmark} \\ \hline
 
\end{tabular}
\end{table}
}}


==> tables/relaxations_alignments.tex <==
\reducemargin{
\arraystretchtable{
\begin{table}[H]\caption{Alignments with corresponding relaxations.}\label{tab:relaxations}
\begin{tabular}{| c | c | c | c |}
\hline
Multitasking & Switching cases & Resource type \\
$L_{mt}=\eventlog{i_s^{\set{d_1}}, \co{i_s}^{\set{d_1}}, \co{i_p}^{\set{d_1}}, i_p^{\set{d_1}}}$
&
$L_{sc}=\eventlog{i_s^{\set{d_1}}, \co{i_s}^{\set{d_2}}, \co{i_p}^{\set{d_1}}, i_p^{\set{d_2}} }$
&
$L_{rt}=\eventlog{i_s^{\set{d_1, n_1}}, i_p^{\set{d_1, n_1}}, i_q^{\set{n_1}}  }$   \\ \hline

\makecell{$\gamma^{(0)}_{mt}$\\
{\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_0-0.pdf}}}
&
\makecell{$\gamma^{(0)}_{sc}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_0-1.pdf}}
&
\makecell{$\gamma^{(0)}_{rt}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_0-2.pdf}} \\ \hline

\makecell{$\gamma^{(1)}_{mt}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_1-0.pdf}}
&
\makecell{$\gamma^{(1)}_{sc}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_1-1.pdf}}
&
$\gamma^{(1)}_{rt} = \gamma^{(0)}_{rt}$    \\ \hline

$\gamma^{(2)}_{mt} = \gamma^{(1)}_{mt}$
&
\makecell{$\gamma^{(2)}_{sc}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_2-1.pdf}}
&
$\gamma^{(2)}_{rt} = \gamma^{(0)}_{rt}$  \\ \hline

$\gamma^{(3)}_{mt} = \gamma^{(1)}_{mt}$
&
$\gamma^{(3)}_{sc} = \gamma^{(2)}_{sc}$
&
\makecell{$\gamma^{(3)}_{rt}$\\
\includegraphics[scale=0.45]{figures2/relaxations_alignments/relax_3-2.pdf}}
\\ \hline

\end{tabular}
\end{table}
}}

==> tables/relaxations_alignments1.tex <==
\reducemargin{
\arraystretchtable{
\begin{table}[H]\caption{Alignments with corresponding relaxations.}\label{tab:relaxations1}
\begin{tabular}{| c | c | c | c |}

\hline
\multicolumn{2}{|c|}{Model move} & \multicolumn{2}{c|}{Log move} \\ \hline
Occupied & Available & Occupied & Available \\ 
$L_{mo}=\eventlog{ \co{o_s}^{d_1}, w_l, i_q^{d_1}, \co{o_c}^{d_1}  }$
&
$L_{ma}=\eventlog{ w_l, i_q^{d_1}  }$
&
$L_{lo}=\eventlog{i_s^{d_1}, i_p^{d_1}, \co{o_s}^{d_1}, i_p^{d_1}, i_q^{d_1}, \co{o_c}^{d_1}}$
&
$L_{la}=\eventlog{i_s^{d_1}, i_p^{d_1}, i_p^{d_1}, i_q^{d_1}}$
\\ \hline
\makecell{$\gamma^{(0)}_{mo}$ \\
\includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_0-0.pdf}}
&
\makecell{$\gamma^{(0)}_{ma}$ \\
\includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_0-1.pdf}}
&
\makecell{$\gamma^{(0)}_{lo}$ \\
\includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_0-2.pdf}}
&
\makecell{$\gamma^{(0)}_{la}$ \\
\includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_0-3.pdf}}\\ \hline

\makecell{$\gamma^{(1)}_{lo}$ \\\includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_1-0.pdf}}
&
$\gamma^{(1)}_{ma} = \gamma^{(0)}_{ma}$
&
$\gamma^{(1)}_{lo} = \gamma^{(0)}_{lo}$
&
\makecell{$\gamma^{(1)}_{la}$ \\ \includegraphics[scale=0.4]{figures2/relaxations_alignments1/1relax_1-3.pdf}}\\ \hline
\end{tabular}
\end{table}
}}

